A theory of cut-restriction: first steps

Cut-elimination is the bedrock of proof theory. It is the algorithm that eliminates cuts from a sequent calculus proof that leads to cut-free calculi and applications. Cut-elimination applies to many logics irrespective of their semantics. Such is its influence that whenever cut-elimination is not provable in a sequent calculus the invariable response has been a move to a richer proof system to regain it. In this paper we investigate a radically different approach to the latter: adapting age-old cut-elimination to restrict the shape of the cut-formulas when elimination is not possible. We tackle the "first level" above cut-free: analytic cuts. Our methodology is applied to the sequent calculi for bi-intuitionistic logic and S5 where analytic cuts are already known to be required. This marks the first steps in a theory of cut-restriction.

==> attempt.tex <==

The above proof of the analytic cut property for $\BiInt$ in not tailored to this specific calculus.
In this section we abstract the proof, and introduce sufficient conditions for a sequent calculus to admit restrictions to analytic cuts.
As an instantiation of this result, we provide an alternative proof of the analytic cut-property for the calculus in~\cite{OhnMat57} for $\SF$.

\begin{definition}
\label{standcalc}
We call any consistent propositional sequent calculus {\em standard} when it satisfies the following conditions:
\begin{enumerate}
\item axioms have the form $p \seq p$, for $p$ variable
\item the calculus contains all structural rules (weakening, exchange and permutation)
\item each logical/modal rule in the calculus
   \begin{enumerate}
      \item has left and right versions, according to the side of the sequent it modifies;
      \item introduces only one connective/modality at a time;
    \item has no side conditions limiting its application (besides, possibly, a condition saying
           that succedents/antecedents are empty or contain only certain formulas, e.g.
           $\Box$-formulas)
      \item has active formulas that are immediate subformulas of the principal
      formula.
   \end{enumerate}
   \end{enumerate}
\end{definition}

The applicability of cut-restriction in a  (standard) sequent calculus relies on the following properties of the calculus:
its rules allow the replacement of cuts by smaller ones (i.e. logical/modal rules
are {\em reductive}), and for each connectives either both the left and right introduction rules are {\em semi-analytic hp-invertible}, or they allow to perform suitable substitutions. Formally,

\begin{definition}
Let $S$ be any standard sequent calculus. We call its (logical or modal) rules
$\{(\star, r)_1, \dots , (\star, r)_n\}$ and
$\{(\star, l)_1,$ $ \dots , (\star, l)_m\}$ for introducing a connective/modality $\star$
{\em reductive}, if for every instance of the rules
the sequent obtained via (cut) on the principal formula of the conclusions
of $(\star, l)_i$ and $(\star, r)_j$ (for each $i= 1, \dots, m$ and $j=1, \dots m$)
can be derived from their premises using (cut) and the structural rules of $S$.
\end{definition}

We write $\prv{X}{\Gamma\Sa\Delta}$ if the sequent $\Gamma\Sa\Delta$ has a proof of height $\le h$ in which all non-analytic cuts have a cut formula in $X$, and wtite $\psf(A)$ to indicate the set of proper subformulas of $A$. Note that if $A$ is atomic, then $\psf(A)=\emptyset$. 

\begin{definition}
A logical rule with principal formula $F$ and conclusion $S_1$ is \emph{ 
semi-analytic hp-invertible} if whenever $\prv{F} S_1$, then $\prv{F \cup\psf(A)} S_i$ for any premise $S_i$ of that rule.
\end{definition}


The reductivity condition is also one of the key (sufficient) conditions to prove cut-elimination in standard calculi (see, e.g.,~\cite{restall:1999a}); the other being the possibility to shift any cut not on the principal formula upwards. 
For cut-restriction we need to relax this second condition, making use of the following notion.

\begin{definition}
Let $S$ be any standard sequent calculus. A rule 
$$\small
\infer[(r)]{\Gamma \seq \Delta}{\Gamma_1 \seq \Delta_1  \dots  & \dots 
 \Gamma_n \seq \Delta_n}$$
is said to be {\em  L-replaceable} (resp. R-replaceable) with a sequent $\Gamma' \seq \Delta'$ if
 for every instance of the rule and any occurrence of the formula $X$, which is not
the principal formula of $(r)$, by cutting possibly multiple times
its conclusion with $\Gamma', X \seq \Delta'$ (resp. $\Gamma' \seq X, \Delta'$) and all corresponding $X$' in its premises (w.r.t. the predecessor relation)
results in a correct application of the rule (possibly using the structural rules).
\end{definition}





\begin{theorem}
In any standard sequent calculus $S$, safisfying the following conditions: 
For every connective/modality $\star(A_1 \dots A_n)$
\begin{enumerate}
    \item its rules are reductive
 \item either its left and right introduction rules are semi-analytic hp-invertible, or they satisfy either for the left or
\begin{itemize}
\item[2.(i)] the left rule (or resp. right) rule introducing $\star(A_1 \dots A_n)$ can be transformed into an axiom by replacing the principal formula  $\star(A_1 \dots A_n)$ with a multiset of formulas (not containing $\top$ or $\bot$)
\item[2.(ii)] every rule is R-replaceble (or resp. L-replaceble) with
the context of the left rule (resp. right) rule introducing $\star(A_1 \dots A_n)$
\item[2.(iii)] all the other calculus rules are L-replaceable  (or resp. L-replaceble)        with the multiset of formulas in 2.(i).
\end{itemize}
\end{enumerate}
cut-restriction holds.
\end{theorem}
\begin{proof}
Let $\delta$ be a proof ending in a non-analytic cut 
\[
\infer[\cut]{\Gamma\Sa \Delta}
	{
	\infer*[\delta_L]{\Gamma\Sa C,\Delta}{}
	&
	\infer*[\delta_R]{\Gamma, C\Sa \Delta}{}
	}
\]
and assume that the subproofs $\delta_L,\delta_R$ are locally analytic. We distinguish cases according to the shape of $C$.
\begin{itemize}
\item The case $C$ is atomic, follows the same pattern as in the proof of $\BiInt$, being
the calculus standard.
\item Let $C$ be a compound formula with most external connective
$\star'(A_1 \dots A_n)$ whose left and right rules are semi-analytic hp-invertible. By using this property, together with reductivity we get a proof of the same end-sequent having only non analytic cuts on $\psf(A_1), \dots ,\psf(A_n)$ which then can be handled by the inductive hypothesis. 
\item Assume now that $C= \star(A_1 \dots A_n)$ and either one of the left or of the right (or both) introduction rules for $\star(A_1 \dots A_n)$ is not semi-analytic hp-invertible. We follow the pattern in the proof for $\BiInt$ of $\impl$. W.l.o.g. we can assume that the proof is irredundant (this property is guaranteed by the presence of contraction). We trace the predecessors of the cut formulas in $\delta_L$ and $\delta_R$. 
Step 1 in the proof goes through using reductivity of the rules and the inductive hypothesis
(on the smaller non-analytic cuts). Step 2 follows by property 2.(i) and 2.(iii). Step 3 follows by property 2.(ii).
\end{itemize}
\end{proof}


==> basicproperties.tex <==
We start by proving some results concerning the admissibility and invertibility of rules in $\BiInt$. These are demonstrated by showing certain simple proof transformations. At the present stage we cannot prove that the transformations preserve local analyticity (although this will follow once the analytic cut property of $\BiInt$ has been established), hence additional care has to be taken of the non-analytic cuts which might be introduced.


%\begin{definition}
%A rule is called \emph{analytic hp-admissible} if whenever its premises have a locally analytic proof of height $h$ then its conclusion has a locally analytic proof of height $\le h$. 
%\end{definition}
%Observe that this is an extension of the standard height-preserving admissible definition to require preservation of locally analytic proofs.
%Not all logical rules can be inverted by preserving locally analytic proofs (analytic hp-invertible rule, see the definition below). This motivates the introduction of the following (terminology and) Definition~\ref{hpi}.

Let us write $\prv{X}{\Gamma\Sa\Delta}$ if the sequent $\Gamma\Sa\Delta$ has a proof of height $\le h$ in in which all non-analytic cuts have a cut formula in $X$. If we set $X=\emptyset$, we recover the notion of locally analytic proof. Moreover let $\psf(A)$ denote the set of proper subformulas of $A$. Note that if $A$ is atomic, then $\psf(A)=\emptyset$. %Furthermore given a $\BiInt$-proof $\gamma$, we denote with $\nac(\gamma)$ the collection of cut formulas occuring in non-analytic cuts in $\gamma$.


%\begin{definition}
%A logical rule with principal formula $A$ is \emph{semi-analytic invertible} if whenever its conclusion has a proof $\gamma$, then each of its premises has a proof $\gamma'$ with $\nac(\gamma')\subseteq\nac(\gamma)\cup\psf(A)$.
%\end{definition}



\begin{lemma}[admissibility and invertibility]
\label{lem:adminv}
\begin{enumerate}
    \item \emph{admissibility of weakening:}\\ If $\prv{X}{\Gamma\Sa\Delta}$ then $\prv{X}{\Gamma,\Sigma\Ra\Delta,\Pi$}.
    \item \emph{invertibility of logical rules:}\\If $\prv{X}{\Gamma\Sa\Delta}$ where $\Gamma\Sa\Delta$ is the conclusion of one of the logical rules $$\{\top_L,\bot_R,\land_L,\land_R,\lor_L,\lor_R\}$$ with principal formula $A$, then $\prv{X\cup\psf(A)}{\Gamma'\Sa\Delta'}$ for any premise $\Gamma'\Sa\Delta'$ of that rule.
    \item \emph{admissibility of left contraction:}\\ If $\prv{X}{\Gamma,A,A\Sa\Delta}$ then $\prv{X\cup\psf(A)}{\Gamma,A\Sa\Delta}$.
    \item \emph{admissibility of right contraction:}\\ If $\prv{X}{\Gamma\Sa A,A,\Delta}$ then $\prv{X\cup\psf(A)}{\Gamma\Sa A,\Delta}$.
\end{enumerate}
\end{lemma}

Note that the (co)implication rules are absent from the Lemma~\ref{lem:adminv}.

%\begin{definition}
%\label{hpi}
%A logical rule with principal formula $F$ is \emph{analytic hp-invertible} (resp. \emph{semi-analytic hp-invertible}) if whenever there is a proof $\delta$ of its conclusion of height $h$, then each of its premises has a proof $\delta'$ of height $\leq h$ which is locally analytic
%(resp. such that
%$NAC(delta’) \subset (NAC(delta) \cup PSF(F))$).
%\end{definition}



%\begin{lemma}
%\label{lem:inv}
%The rules $\top_L$ and \bot_R$ are %analytic hp-invertible in $\BiInt$, and
%\[
%\infer[\weak]{\Gamma,\Sigma\Sa\Delta,\Pi}
%	{
%	\Gamma\Sa\Delta
%	}
%	\]
%is analytic hp-admissible in $\BiInt$.
%\end{lemma}
%\begin{proof}
%... TO BE DONE ...
%\end{proof}

% Due to the fact that the logical rules $\land_R, \lor_L, \imp_L, \coimp_R$ of $\BiInt$ are only semi-analytic hp-invertible (see below), we cannot require the contraction rule to be analytic hp-admissible. Still,
% as shown in the following lemma, its admissibility results in a proof with non-analytic cuts of 
% limited size.

% \begin{lemma}
% \label{lem:semi-inv}
% \begin{enumerate}
% \item\label{hpadmissible}
% Whenever the premise of the contraction rule
% \[
% \infer[\contr]{\Gamma,\Sigma\Sa\Delta,\Pi}
% 	{
% 	\Gamma,\Sigma,\Sigma\Sa\Delta,\Delta,\Pi
% 	}
% \]
% has a proof $\delta$ in $\BiInt$ of height $\le h$, then its premise has a proof $\delta'$ of height $\leq h$ such that
% $NAC(delta’) \subset (NAC(delta) \cup PSF(\Sigma \cup \Delta))$)
% %has a proof of height $\le h$ whose only non-analytic cuts are on strict subformulas of $\Sigma \cup \Delta$ 
% (semi-analytic hp-admissible).
% \item\label{hpinvertible}
% The following rules are semi-analytic hp-invertible in $\BiInt$:
% \[
% \land_L,\land_R,\lor_L\text{ and }\lor_R
% \]
% \end{enumerate}
% \end{lemma}
\begin{proof}
By induction on the height of proofs. The admissibility of weakening goes through without complications. The invertibility of logical rules and the admissibility of contraction have to be proved simultaneously due to some inderdependencies.

We discuss some representative cases and refer the reader to the Appendix for the full proof.
%
Due to the presence of analytic cuts, we need to argue on   
the admissibility and invertibility of all the rules
simultaneously (and indicate with \textit{IH cntr} and \textit{IH inv} the induction hypothesis on  semi-analytic hp-admissibility and -invertibility respectively).
%Since there is some interdependency, one must argue on all the rules in (\ref{hpadmissible}) and (\ref{hpinvertible}) simultaneously.
%
%For $\weak$ the argument is straightforward. 

For the admissibility of $\contr$ we illustrate the situation when we have a locally analytic proof ending as follows:
\begin{center}
\AxiomC{$\Gamma \Ra A, A\wedge B, \Delta$}
\AxiomC{$\Gamma \Ra B, A \wedge B, \Delta$}
\RightLabel{$\imp_L$}
\BinaryInfC{$\Gamma \Ra A\wedge B, A\wedge B, \Delta$}
\DisplayProof
\end{center}
The claim holds by applying the \textit{IH inv} to $A \wedge B$ (resulting in a proof of height $\leq h-1$ whose only non-analytic cuts are on $A$ and $B$), the  \textit{IH cntr} (resulting in a proof having the same property) and an application of $\impl_L$.

\marginpar{I did not change it but for me it can be handle with the semi-invertibility of the standard rule}
A slightly different case is when we have a locally analytic proof ending as follows:
\begin{center}
\AxiomC{$\Gamma, A\imp B, A\imp B \Ra \Delta, A$}
\AxiomC{$\Gamma, A\imp B, A\imp B, B\Ra \Delta$}
\RightLabel{$\imp_L$}
\BinaryInfC{$\Gamma, A\imp B, A\imp B \Ra \Delta$}
\DisplayProof
\end{center}
We proceed as follows: 
%Here \textit{IH cntr} and \textit{IH inv} refer to the induction hypothesis on locally analytic hp-admissibility and -invertibility respectively.
\begin{center}
\AxiomC{$\Gamma, A\imp B, A\imp B \Ra \Delta, A$}
\RightLabel{IH cntr}
\dashedLine
\UnaryInfC{$\Gamma, A\imp B\Ra \Delta, A$}
%
\AxiomC{$\Gamma, A\imp B, A\imp B, B\Ra \Delta$}
\RightLabel{IH cntr}
\dashedLine
\UnaryInfC{$\Gamma, A\imp B, B\Ra \Delta$}
%
\RightLabel{$\imp_L$}
\BinaryInfC{$\Gamma, A\imp B\Ra \Delta$}
\DisplayProof
\end{center}
As another example, let us turn to establishing semi-analytic hp-invertibility.
In the case of $\land_L$ we need to prove locally analytic hp-admissibility of the rule
\[
\infer{\Gamma,A,B\Sa\Delta}{\Gamma,A\land B\Sa\Delta}
\]
We consider the last rule applied in the locally analytic proof of $\Gamma,A\land B\Sa\Delta$. The only interesting case is when this rule is an analytic cut, as in:
\[
	\infer[cut]{\Gamma,A\land B\Sa\Delta}
		{
		\Gamma,A\land B\Sa C,\Delta
		&
		\Gamma,A\land B,C\Sa \Delta
		}
\]
If $C\neq A\land B$ then it suffices to apply the IH to the premises and proceed as follows
\[
\infer[cut]{\Gamma,A,B\Sa\Delta}
	{
	\Gamma,A,B\Sa C,\Delta
	&
    \Gamma,A,B,C\Sa\Delta
	}
\]
The strategy does not work anymore if $C=A\land B$ as the cut may cease to be analytic and is not on a strict subformula of $A \wedge B$. In that case, by \textit{IH cntr} on the right premise we obtain $\Gamma,A\land B\Sa\Delta$. Now $\Gamma,A,B\Ra\Delta$ follows from \textit{IH inv}.

A case, which shows the need of relaxing the requirement of local analiticity for the proofs of the premises, is the $\wedge_R$ rule.
Assume that the last rule applied is an analytic cut, as in:
\[
	\infer[cut]{\Gamma\Sa A \wedge B, \Delta}
		{
		\Gamma \Sa A \wedge B, C,\Delta
		&
		\Gamma, C\Sa, A \wedge B, \Delta
		}
\]
Being the cut analytic, $C$ is a subformula of $\{ \Gamma\cup \{A \wedge B\} \cup \Delta\}$. If $C = A \wedge B$, as in the previous case, we get the
desired sequent 
by \textit{IH cntr} followed by
\textit{IH inv}. Assuming  that $C\neq A\land B$. By \textit{IH inv} applied to the left premise we get
$\Gamma \Sa A, C,\Delta$ and $\Gamma \Sa B, C,\Delta$ and
from the right premise we get 
$\Gamma, C\Sa, A, \Delta$ and $\Gamma, C\Sa, B, \Delta$.
By cutting on $C$
we get $\Gamma \Sa A, \Delta$ and $\Gamma \Sa B,\Delta$. We reason on $C$: if $C$ is a subformula of $\{ \Gamma \cup \Delta\}$ then the proof is locally analytic. However, when $C = A$, then the proof of
$\Gamma \Sa B,\Delta$ is not locally analytic anymore but the only non-analytic cut that the proof contains is a cut on $A$, which is a strict subformula of $A \wedge B$. The case $C = B$ is symmetric.
\qed\end{proof}

\begin{remark}\label{rem-variant}
\marginpar{If we keep the standard rules, no need if it}
The modified version of the $\imp_L$ rule we are using (cfr. Figure~\ref{fig:BiInt}) is motivated by the obstacle we encountered 
%We encounter the following obstacle 
while attempting to establish that the standard $\imp_L$ rule (below) is locally analytic hp-invertible in the right premise
\begin{center}
\AxiomC{$\Gamma, A\imp B\Ra A, \Delta$}
\AxiomC{$\Gamma, B\Ra\Delta$}
\BinaryInfC{$\Gamma,A\imp B\Ra\Delta$}
\DisplayProof
\end{center}
Indeed given a proof of $\Gamma,A\imp B\Ra\Delta$ we would like be to obtain a proof of $\Gamma,B\Ra\Delta$ by induction on the height of the former. However consider the case in which the last rule in the proof of $\Gamma, A\imp B\Ra\Delta$ is a cut on~$A$; its premises are $\Gamma, A\imp B\Ra \Delta, A$ and $\Gamma, A\imp B, A\Ra \Delta$. By the induction hypothesis we would obtain $\Gamma, B\Ra \Delta, A$ and $\Gamma, B, A\Ra\Delta$. A cut would give us $\Gamma, B\Ra\Delta$ but this cut might not be analytic, and hence the argument breaks down.

%This illustrates the particular care that is required when reasoning about analytic rules.

Had we used the standard $\imp_L$ rule then the analytic height-preserving admissibility of contraction would have required analytic height-preserving invertibility of $\imp_L$ (to tackle $\Gamma, A\imp B, A\imp B\Ra\Delta$). Having seen that this result is problematic to obtain we used a variant of the standard rule. We can nevertheless recover the analytic cut property for the original calculus in~\cite{Rau74}, as explained in the proof of Thm~\ref{thm-main}.
\end{remark}





==> k5.tex <==
\section{$K5$ incomplete}

The sequent calculus for $K5$ extends the sequent calculus $LK$ for classical propositional logic with the following rule:
\begin{center}
\AxiomC{$\Gamma\Ra \Box\Theta, A$}
\RightLabel{$5$}
\UnaryInfC{$\Box\Gamma\Ra \Box\Theta, \Box A$}
\DisplayProof
\end{center}
The $5$ axiom is $\lnot\Box p\imp \Box\lnot\Box p$.

Takano (A Modified Subformula Property for the Modal Logics K5 and K5D) shows that every provable sequent has a proof built from formulas that are $K5$-subformulas of the endsequent i.e. subformulas of the endsequent, or $\Box\lnot\Box B$ or $\lnot\Box B$ such that $\Box B$ is an internal subformula (i.e. itself nested under a $\Box$) of the endsequent.

The critical case is the following. As always, we first identify the predecessors of the cut-formulas. For simplicity we suppose a single critical inference in each premise.
\begin{center}
\AxiomC{$\Gamma'\Ra \Box\Theta',A$}
\RightLabel{$5$}
\UnaryInfC{$\Box\Gamma'\Ra \Box\Theta',\Box A$}
\noLine
\UnaryInfC{$\leftpremise$}
\noLine
\UnaryInfC{$\Gamma\Ra \Theta, \Box A$}
%
\AxiomC{$A, X'\Ra \Box Y', B$}
\RightLabel{$5$}
\UnaryInfC{$\Box A, \Box X'\Ra \Box Y', \Box B$}
\noLine
\UnaryInfC{$\rightpremise$ no $5$ rule}
\noLine
\UnaryInfC{$\Box A, X\Ra Y$}
%
\RightLabel{cut}
\BinaryInfC{$\Gamma, X\Ra \Theta, Y$}
\DisplayProof
\end{center}
We proceed as follows.
\begin{center}
\begin{footnotesize}
\AxiomC{$\Gamma\Ra\Theta,\lnot\Box\Theta'$}
%
\AxiomC{}
\UnaryInfC{$\lnot\Box\Theta'\Ra\Box\lnot\Box\Theta'$}
%
\AxiomC{$\Gamma\Ra\Theta,\Box\Gamma'$}
%
\AxiomC{$\Gamma'\Ra \Box\Theta',A$}
\AxiomC{$A, X'\Ra \Box Y', B$}
\RightLabel{cut}
\BinaryInfC{$\Gamma', X'\Ra \Box\Theta', \Box Y', B$}
\RightLabel{$\lnot R$}
\UnaryInfC{$\Gamma', X', \lnot\Box\Theta'\Ra  \Box Y', \Box B$}
\RightLabel{$5$}
\UnaryInfC{$\Box\Gamma', \Box X', \Box\lnot\Box\Theta'\Ra  \Box Y', \Box B$}
%
\RightLabel{cut}
\BinaryInfC{$\Gamma, \Box X', \Box\lnot\Box\Theta'\Ra  \Box Y', \Box B$}
\RightLabel{cut}
\BinaryInfC{$\Gamma, \Box X', \lnot\Box\Theta'\Ra  \Box Y', \Box B$}
%
\RightLabel{cut}
\BinaryInfC{$\Gamma, \Box X'\Ra  \Box Y', \Box B$}
\noLine
\UnaryInfC{$+\rightpremise$}
\noLine
\UnaryInfC{$\Gamma, X\Ra  \Box Y$}
\DisplayProof
\end{footnotesize}
\end{center}
It's not enough to choose a topmost cut that is not a $K5$-subformula. We also need that $\Box\Theta'$ is an (internal) subformula of the endsequent, since the above transformation cuts on $\Box\lnot\Box\Theta'$ and $\lnot\Box\Theta'$.

If we can restrict antecedent formulas to subformulas, or $\lnot\Box B$ ($\Box B$ is a subformula), or $\Box\lnot\Box B$ at an initial sequent ($\Box B$ is a subformula) then we might be fine, but I'm not sure how we can do this.



==> oldbasicproperties.tex <==
We start by proving fairly standard admissibility/invertibility results in the context of
locally analytic proofs.

\begin{definition}
A rule is called \emph{locally analytic hp-admissible} if whenever its premises have a locally analytic proof of height $h$ then its conclusion has a locally analytic proof of height $\le h$. 
\end{definition}
Observe that this is an extension of the standard height-preserving admissible definition to require preservation of locally analytic proofs.
\begin{definition}
A rule is \emph{locally analytic hp-invertible} if each of the unary rules going from conclusion to a premise is locally analytic hp-admissible.
\end{definition}


\begin{lemma}%[admissible rules of $\BiInt$]\mbox{}
\label{lem:adm}
\begin{enumerate}
\item\label{hpadmissible}
The following rules are locally analytic hp-admissible in $\BiInt$:
\[
\infer[\weak]{\Gamma,\Sigma\Sa\Delta,\Pi}
	{
	\Gamma\Sa\Delta
	}
\qquad
\infer[\contr]{\Gamma,\Sigma\Sa\Delta,\Pi}
	{
	\Gamma,\Sigma,\Sigma\Sa\Delta,\Delta,\Pi
	}
\]
\item\label{hpinvertible}
The following rules $\BiInt$ are locally analytic hp-invertible in $\BiInt$:
\[
\top_L,\bot_R,\land_L,\land_R,\lor_L\text{ and }\lor_R
\]
\end{enumerate}


%\[
%\infer[\top^*]{\Gamma\Sa\Delta}
%	{
%	\Gamma,\top\Sa\Delta
%	}
%\qquad
%\infer[\bot^*]{\Gamma\Sa\Delta}
%	{
%	\Gamma\Sa\bot,\Delta
%	}
%\]
%\[
%\infer[\land_L^*]{\Gamma,A,B\Sa\Delta}
%	{
%	\Gamma,A\land B\Sa\Delta
%	}
%\qquad
%\infer[\land_R^*]{\Gamma\Sa A,\Delta}
%	{
%	\Gamma\Sa A\land B,\Delta
%	}
%\qquad
%\infer[\land_R^*]{\Gamma\Sa B,\Delta}
%	{
%	\Gamma\Sa A\land B,\Delta
%	}
%\]
%\[
%\infer[\lor_L^*]{\Gamma,A\Sa\Delta}
%	{
%	\Gamma,A\lor B\Sa\Delta
%	}
%\qquad
%\infer[\lor_L^*]{\Gamma,B\Sa\Delta}
%	{
%	\Gamma,A\lor B\Sa\Delta
%	}
%\qquad
%\infer[\lor_R^*]{\Gamma\Sa A,B,\Delta}
%	{
%	\Gamma\Sa A\lor B,\Delta
%	}
%\]
\end{lemma}
\begin{proof}
By induction on the height of a proof deriving the premise of the respective rule. We only discuss two representative cases and refer the reader to the Appendix for the full proof.
%
Due to the presence of analytic cuts, we need to argue on 
all the rules 1. and 2. simultaneously (and indicate with \textit{IH cntr} and \textit{IH inv} the induction hypothesis on locally analytic hp-admissibility and -invertibility respectively).
%Since there is some interdependency, one must argue on all the rules in (\ref{hpadmissible}) and (\ref{hpinvertible}) simultaneously.
%
%For $\weak$ the argument is straightforward. 

For the admissibility of $\contr$ we illustrate the situation when we have a locally analytic proof ending as follows:
\begin{center}
\AxiomC{$\Gamma, A\imp B, A\imp B \Ra \Delta, A$}
\AxiomC{$\Gamma, A\imp B, A\imp B, B\Ra \Delta$}
\RightLabel{$\imp_L$}
\BinaryInfC{$\Gamma, A\imp B, A\imp B \Ra \Delta$}
\DisplayProof
\end{center}
We proceed as follows: 
%Here \textit{IH cntr} and \textit{IH inv} refer to the induction hypothesis on locally analytic hp-admissibility and -invertibility respectively.
\begin{center}
\AxiomC{$\Gamma, A\imp B, A\imp B \Ra \Delta, A$}
\RightLabel{IH cntr}
\dashedLine
\UnaryInfC{$\Gamma, A\imp B\Ra \Delta, A$}
%
\AxiomC{$\Gamma, A\imp B, A\imp B, B\Ra \Delta$}
\RightLabel{IH cntr}
\dashedLine
\UnaryInfC{$\Gamma, A\imp B, B\Ra \Delta$}
%
\RightLabel{$\imp_L$}
\BinaryInfC{$\Gamma, A\imp B\Ra \Delta$}
\DisplayProof
\end{center}
As another example, let us turn to establishing locally analytic hp-invertibility. In the case of $\land_L$ we need to prove locally analytic hp-admissibility of the rule
\[
\infer{\Gamma,A,B\Sa\Delta}{\Gamma,A\land B\Sa\Delta}
\]
We consider the last rule applied in the locally analytic proof of $\Gamma,A\land B\Sa\Delta$. The only interesting case is when this rule is an analytic cut, as in:
\[
	\infer[cut]{\Gamma,A\land B\Sa\Delta}
		{
		\Gamma,A\land B\Sa C,\Delta
		&
		\Gamma,A\land B,C\Sa \Delta
		}
\]
If $C\neq A\land B$ then it suffices to apply the IH to the premises and proceed as follows
\[
\infer[cut]{\Gamma,A,B\Sa\Delta}
	{
	\Gamma,A,B\Sa C,\Delta
	&
    \Gamma,A,B,C\Sa\Delta
	}
\]
The strategy does not work anymore if $C=A\land B$ as the cut may cease to be analytic. In that case, by \textit{IH cntr} on the right premise we obtain $\Gamma,A\land B\Sa\Delta$. Now $\Gamma,A,B\Ra\Delta$ follows from \textit{IH inv}.
\qed\end{proof}

\begin{remark}\label{rem-variant}
The modified version of the $\imp_L$ rule we are using (cfr. Figure~\ref{fig:BiInt}) is motivated by the obstacle we encountered 
%We encounter the following obstacle 
while attempting to establish that the standard $\imp_L$ rule (below) is locally analytic hp-invertible in the right premise
\begin{center}
\AxiomC{$\Gamma, A\imp B\Ra A, \Delta$}
\AxiomC{$\Gamma, B\Ra\Delta$}
\BinaryInfC{$\Gamma,A\imp B\Ra\Delta$}
\DisplayProof
\end{center}
Indeed given a proof of $\Gamma,A\imp B\Ra\Delta$ we would like be to obtain a proof of $\Gamma,B\Ra\Delta$ by induction on the height of the former. However consider the case in which the last rule in the proof of $\Gamma, A\imp B\Ra\Delta$ is a cut on~$A$; its premises are $\Gamma, A\imp B\Ra \Delta, A$ and $\Gamma, A\imp B, A\Ra \Delta$. By the induction hypothesis we would obtain $\Gamma, B\Ra \Delta, A$ and $\Gamma, B, A\Ra\Delta$. A cut would give us $\Gamma, B\Ra\Delta$ but this cut might not be analytic, and hence the argument breaks down.

%This illustrates the particular care that is required when reasoning about analytic rules.

Had we used the standard $\imp_L$ rule then the analytic height-preserving admissibility of contraction would have required analytic height-preserving invertibility of $\imp_L$ (to tackle $\Gamma, A\imp B, A\imp B\Ra\Delta$). Having seen that this result is problematic to obtain we used a variant of the standard rule. We can nevertheless recover the analytic cut property for the original calculus in~\cite{Rau74}, as explained in the proof of Thm~\ref{thm-main}.
\end{remark}


%We will make heavy use of Lemma~\ref{lem:adm}, but it is important to note that the admissible rules are never formally added to the calculus.  When $\gamma$ is a locally analytic proof of some sequent $S$ and the rule $S/S'$ is admissible by Lemma~\ref{lem:adm}, we may symbolically write\marginpar{use dashed line}
%\[
%\infer={S'}{\infer*[\gamma]{S}{}}
%\]
%to denote the (or any) locally analytic proof guaranteed to exist by Lemma~\ref{lem:adm} whose endsequent is $S'$ and whose height does not exceed that of $\gamma$.


%\section{Proof idea}
%The so-called \emph{principal cases} of cut reduction are those where the cut formula is principal in both premises of cut, e.g.
%\[
%\infer[\cut]{\Gamma\Sa\Delta}
%	{
%	\infer[\imp_R]{\Gamma\Sa A\imp B,\Delta}
%		{
%		\infer*[\delta_1]{\Gamma,A\Sa B}{}
%		}
%	&
%	\infer[\imp_L]{\Gamma,A\imp B\Sa\Delta}
%		{
%		\infer*[\epsilon_1]{\Gamma,A\imp B\Sa A,\Delta}{}
%		&
%		\infer*[\epsilon]{\Gamma,B\Sa\Delta}{}
%		}
%	}
%\]
%In this case the canonical cut reduction is the following:
%\[
%\infer[\cut]{\Gamma\Sa\Delta}
%	{
%	\infer[\cut]{\Gamma\Sa A,\Delta}
%		{
%		\infer[\imp_R]{\Gamma\Sa A\imp B,\Delta}
%			{
%			\infer*[\delta_1]{\Gamma,A\Sa B}{}
%			}
%		&
%		\infer*[\epsilon_1]{\Gamma,A\imp B\Sa A,\Delta}{}
%		}
%	&
%	\infer[\cut]{\Gamma,A\Sa\Delta}
%		{
%		\infer*[\delta_1]{\Gamma,A\Sa B}{}
%		&
%		\infer*[\epsilon]{\Gamma,B\Sa\Delta}{}
%		}
%	}
%\]
%The non-principal cases of cut reduction deal with how to achieve the principal case. There are two methods:
%\begin{enumerate}
%\item Shifting the cut upwards over both premises until one reaches a principal case
%\item Globally rewriting the proof such that the cut formula becomes principal in both premises.
%\end{enumerate}
%The second method works if the rule pertaining to the main connective of the cut formula is invertible. 
%
%Both methods fail in the case of $\BiInt$.  In the following we describe a different method of cut reduction.  This method will not---and cannot---eliminate all cuts, but it will reduce all cuts to analytic ones.
%
%The method is quite similar to the reduction in the principal case, only that we no longer require the cut formula to be principal directly above the cut.  Instead, we trace the cut formula upwards in both branches until it becomes principal:
%
%\[
%\infer[\cut]{\Gamma\Sa\Delta}
%	{
%	\infer*[\delta]{\Gamma\Sa A\imp B,\Delta}
%	{
%		\infer[\imp_R]{\Gamma'\Sa A\imp B,\Delta'}
%			{
%			\infer*[\delta_1]{\Gamma',A\Sa B}{}
%		}
%	}
%	&
%	\infer*[\epsilon]{\Gamma,A\imp B\Sa\Delta}
%	{
%	\infer[\imp_L]{\Gamma'',A\imp B\Sa\Delta''}
%		{
%		\infer*[\epsilon_1]{\Gamma'',A\imp B\Sa A,\Delta''}{}
%		&
%		\infer*[\epsilon_2]{\Gamma'',B\Sa\Delta''}{}
%		}
%	}
%	}
%\]
%By making cuts between the subderivations $\delta_1,\epsilon_1$ and $\epsilon_2$ mimicking the principal case reduction one obtains a proof $c(\delta_1,\epsilon_1,\epsilon_2)$ of the sequent $\Gamma'',\Gamma'\Sa\Delta''$ [TODO: picture if necessary]. This is exactly the conclusion of $\imp_L$ in the above proof figure with $\Gamma'$ substituted for $A\imp B$.  The idea is now to extend this substitution to the lower part of the proof, that is, to $\delta$ and $\epsilon$.  Assuming for simplicity that $\Gamma'$ consists of a single formula,  we obtain the following derivation:
%\[
%\infer[\cut]{\Gamma\Sa\Delta}
%	{
%	\infer*[\delta\text{ [subst. $\Gamma'$ for $A\imp B$]}]{\Gamma\Sa\Gamma',\Delta}
%		{
%		\Gamma'\Sa\Gamma',\Delta'
%		}
%	&
%	\infer*[\epsilon\text{ [subst. $\Gamma'$ for $A\imp B$]}]{\Gamma,\Gamma'\Sa\Delta}
%		{
%		\infer*[c(\delta_1,\epsilon_1,\epsilon_2)]{\Gamma'',\Gamma'\Sa\Delta''}
%			{
%			}
%		}
%	}
%\]
%Herein the cut on $A\imp B$ has been replaced by a cut on $\Gamma'$.  
%
%It is not immediately clear in which sense this proof transformation constitutes a \emph{reduction}.  We will argue for the following: If the cut on $A\imp B$ is the lowermost non-analytic cut in the original proof and if the proof is free from certain redundancies, then
%\begin{itemize}
%\item either $\Gamma'$ is a proper subformula of $A\imp B$, or
%\item $\Gamma'$ is a subformula of $\Gamma\cup\Delta$.
%\end{itemize}
%In the first case the introduced cut on $\Gamma'$ has smaller degree, and using an inductive argument we may therefore assume that it can be reduced. In the second case, the cut on $\Gamma'$ is analytic, and we just leave it as it is.
%
%A complication arises because analytic cuts in $\delta$ and $\epsilon$ may cease to be analytic after the substitution. But again, we will argue that this is only the case if they were cuts on proper subformulas of $A\imp B$, and thus reducible by induction hypothesis.
%
%Another conceptionally less interesting complication comes from the possibility that there can be multiple instances of $\imp_L$ and $\imp_R$ introducing the cut formula, and from the possibility that $\Gamma'$ contains more than one formula. These are dealt with by \ldots




==> oldintro.tex <==

\section*{Tentative titles}

Towards cut-reduction? Reducing cuts in Bi-Intuitionistic Logic?

Cut-reduction: the first step [our technical result is very specific, so we need to draw attention to the big idea behind it]

\section{Introduction}

[draft, obviously citations to be filled in]

Cut-elimination is the fundamental result of proof theory. At its heart, it is an algorithm for transforming a proof into an analytic proof by eliminating the most common source of non-analyticity: the the cut-rule. Analytic proofs are better behaved and more amenable to meta-theoretic investigation as the space of possible proofs is greatly constrained. This has been exploited in a myriad of ways: Gentzen's original motivation was a finitistic proof of the consistency of arithmetic; this paved the way to the development of ordinal analysis; the cut-free calculi that are the offspring of cut-elimination are central in structural proof theory where they are used to investigate the underlying logic; automated theorem proving and normalisation in process calculi are a few of the many areas impacted by this result.

Gentzen's cut-elimination arguments are well-known to the logic community: stepwise transformations replace cut-rules in the proof by simpler cut-rules, and an appeal to (transfinite) induction ultimately yields a cut-free proof.

Let us pick up the story in the decades following Gentzen's seminal result from the 1930s. 
Cut-elimination was originally proved for sequent calculi for classical and intuitionistic logic. 
The programme of developing cut-free calculi via cut-elimination was soon extended to non-classical logics, notably modal logics. The first significant obstacle was encountered in the 1950s: how to eliminate cuts in the proof calculus for the modal logic $S5$? Mints found a solution in the 1960s by extending the metalanguage of the proof calculus from Gentzen's sequent calculus to essentially what is today called the hypersequent calculus. Hypersequent calculi were rediscovered independently by Avron~\cite{Avr87} and Pottinger~\cite{Pot83} in the 1980s who used it to obtain cut-elimination for relevant and modal logics. The floodgates had been opened: whenever Gentzen-style argument fail to deliver cut-elimination for a logic of interest, the standard response in structural proof theory is to look (or invent) a new proof formalism by extending the metalanguage of the sequent calculus such that cut-elimination \textit{does} hold. More than a dozen proof formalisms have been introduced in this way.

A question never addressed in all this time is whether it is possible to adapt cut-elimination to simplify cuts that are not eliminable. This is \textbf{cut-reduction}.

Ciabattoni \textit{et al.} presented an indirect proof-of-principle by transforming cut-free hypersequent calculi for substructural, intermediate, and modal logics to sequent calculi with cut-formulas that were parametric on the end formula (not necessarily subformulas). The space of possible sequent calculus proofs was still constrained enough to obtain meta-theoretic results such as decidability, complexity, and logical embeddings.
Cut-reduction was mentioned but left open. 

In this paper we establish cut-reduction in the context of bi-intuitionistic logic by showing how adapt the cut-elimination arguments to stepwise transform a proof with arbitrary cuts to a proof with analytic cuts.

We emphasise that completeness of the sequent calculus with analytic cuts for bi-intuitionistic logic was already shown in Kowalski and Ono\cite{KowOno17}, itself based on Takano's proof of analytic cut completeness for $S5$~\cite{Tak92} (see also Fitting's semantic arguments~\cite{Fit78} for other modal logics). The key point of this work is obtaining this result as an adaptation of Gentzen's cut-elimination. It is a first foray towards a theory of cut-reduction.


\subsection*{From Cut-Elimination to Cut-Reduction}
%Extending Gentzen's cut-elimination arguments}

Gentzen defines two types of local transformations to eliminate cut: \textit{permutation reductions} permute a cut upwards until the cut-formula is principal in the left and right premises of the cut, and  \textit{principal reduction} replace the cut with strictly simpler cuts.

Why does cut-elimination fail for some sequent calculi? It can be hard to find a suitable principal reduction when the sequent rules are non-standard and contain some syntactic peculiarity. A good example is the modal rule in provability logic $GL$: the change in polarity of the so-called diagonal formula from conclusion to premise forces a highly intricate and customised principal reduction.
Here we will consider cut-reduction in the context of standard sequent calculi: the sequent rules are standard and so the principal reductions are unproblematic. Hence we shift our attention to permutation reductions. 

The reason for the failure of permutation reductions is subtle. Consider the elimination of the cut below in Maehara's intuitionistic propositional calculus (see~\cite{Takeuti:87}). This is a multiple-conclusion calculus (i.e. sequents have the form $\Gamma\Ra\Delta$ for multisets $\Gamma,\Delta$) and \textit{the succedent of the ${\imp}R$ rule is permitted no context}.
\begin{equation}\label{original-cut}
\text{
\AxiomC{$\eta$}
\noLine
\UnaryInfC{$X \Ra Y, A\imp B$}
%
\AxiomC{$\pi$}
\noLine
\UnaryInfC{$U, A\imp B, C \Ra D$}
\UnaryInfC{$U, A\imp B \Ra C\imp D$}
\RightLabel{cut}
\BinaryInfC{$X, U \Ra Y, C\imp D$}
\DisplayProof
}
\end{equation}
If we permuted the cut upwards in the right premise (a permutation reduction) we reach the following situation.
\begin{center}
\AxiomC{$\eta$}
\noLine
\UnaryInfC{$X \Ra Y, A\imp B$}
%
\AxiomC{$\pi$}
\noLine
\UnaryInfC{$U, A\imp B, C \Ra D$}
\RightLabel{cut}
\BinaryInfC{$X, U , C \Ra Y, D$}
\DisplayProof
\end{center}
However, we cannot obtain $X, U\Ra Y, C\imp D$ from $X, U , C \Ra Y, D$ because the presence of~$Y$ blocks the ${\imp}R$ rule. Instead of permuting upwards in the right premise, a solution is found by first permuting the cut upwards in the left premise, until the succedent $A\imp B$ becomes principal. Let us \textit{trace upwards the formula $A\imp B$ in the left premise} to identify where it is introduced (principal). For simplicity, let us assume that there is exactly one such `critical sequent' witnessing the introduction of $A\imp B$:
\begin{center}
\AxiomC{$X', A \Ra B$}
\UnaryInfC{$X' \Ra A\imp B$}
\noLine
\UnaryInfC{$\eta$}
\noLine
\UnaryInfC{$X \Ra Y, A\imp B$}
%
\AxiomC{$U, A\imp B, C \Ra D$}
\UnaryInfC{$U, A\imp B \Ra C\imp D$}
\RightLabel{cut}
\BinaryInfC{$X, U \Ra Y, C\imp D$}
\DisplayProof
\end{center}
Permuting the cut upwards in the left premise we reach the following situation.
\begin{center}
\AxiomC{$X', A \Ra B$}
\UnaryInfC{$X' \Ra A\imp B$}
%
\AxiomC{$U, A\imp B, C \Ra D$}
\UnaryInfC{$U, A\imp B \Ra C\imp D$}
\RightLabel{cut}
\BinaryInfC{$X', U \Ra Y, C\imp D$}
\noLine
\UnaryInfC{$+\eta+$}
\noLine
\UnaryInfC{$X, U \Ra Y, A\imp B, C\imp D$}
\DisplayProof
\end{center}
Here $+\eta+$ indicates that the sequents in the featured branch in $\eta$ are enriched with additional multisets in the antecedent and succedent. Note that $+\eta+$ is well-defined because no ${\imp}R$ could have occurred on this branch in $\eta$ (we traced the $A\imp B$ occurring in the succedent and this would block the ${\imp}R$ rule).
What next? Now \textit{trace upwards the formula $A\imp B$ in the right premise} of cut:
\begin{equation}\label{right-premise-trace}
\text{
\AxiomC{$X', A \Ra B$}
\UnaryInfC{$X' \Ra A\imp B$}
%
\AxiomC{$U', A\imp B \Ra V', A$}
\AxiomC{$U', B \Ra V'$}
\BinaryInfC{$U', A\imp B \Ra V'$}
\noLine
\UnaryInfC{$\pi$}
\noLine
\UnaryInfC{$U, A\imp B \Ra C\imp D$}
\RightLabel{cut}
\BinaryInfC{$X', U \Ra Y, C\imp D$}
\noLine
\UnaryInfC{$+\eta+$}
\noLine
\UnaryInfC{$X, U \Ra Y, A\imp B, C\imp D$}
\DisplayProof
}
\end{equation}
Permuting the cut upwards in the right premise we reach
\begin{center}
\AxiomC{$X', A \Ra B$}
\UnaryInfC{$X' \Ra A\imp B$}
%
\AxiomC{$U', A\imp B \Ra V', A$}
\AxiomC{$U', B \Ra V'$}
\BinaryInfC{$U', A\imp B \Ra V'$}
%
\RightLabel{cut}
\BinaryInfC{$X', U' \Ra V'$}
\noLine
\UnaryInfC{$+\pi$}
\noLine
\UnaryInfC{$X', U, C \Ra D$}
\UnaryInfC{$X', U \Ra C\imp D$}
\noLine
\UnaryInfC{$+\eta+$}
\noLine
\UnaryInfC{$X, U \Ra Y, C\imp D$}
\DisplayProof
\end{center}
The $+\pi$ indicates that the sequents along the featured branch in $\pi$ are enriched with an additional multiset in the antecedent. Note that $+\pi$ is well-defined because the ${\imp}R$ restriction applies only to the succedent.
The cut-formula in the above cut is principal in both the left and right premise. This is precisely the moment to use the principal reduction:
\begin{equation}\label{cut-elim-principal}
\text{
\AxiomC{$X', A \Ra B$}
\UnaryInfC{$X' \Ra A\imp B$}
%
\AxiomC{$U', A\imp B \Ra V', A$}
\BinaryInfC{$X', U', \Ra V', A$}
%
\AxiomC{$X', A \Ra B$}
\BinaryInfC{$X',X', U', \Ra V', B$}
%
\AxiomC{$U', B \Ra V'$}
\BinaryInfC{$X',X', U', U'\Ra V', V'$}
\RightLabel{ctr}
\UnaryInfC{$X', U'\Ra V'$}
\noLine
\UnaryInfC{$+\pi$}
\noLine
\UnaryInfC{$X', U, C \Ra D$}
\UnaryInfC{$X', U \Ra C\imp D$}
\noLine
\UnaryInfC{$+\eta+$}
\noLine
\UnaryInfC{$X, U \Ra Y, C\imp D$}
\DisplayProof
}
\end{equation}
Notice that we could have proceeded from the original proof (\ref{original-cut}) to this in a single transformation by directly tracing the $A\imp B$ upwards in both premises. Even so, the correctness of the transformation relies crucially on $+\pi$ being well defined (and implicitly, a suitable strategy for the permutation reductions).

A calculus for bi-intuitionistic logic is obtained from the Maehara calculus by extending the intuitionistic language with \textit{coimplication}~$\coimp$ and adding the following rules:
\begin{center}
\begin{tabular}{c@{\hspace{1cm}}c}
\AxiomC{$A\Ra X,B$}
\RightLabel{$\coimp$L}
\UnaryInfC{$A\coimp B\Ra X$}
\DisplayProof
&
\AxiomC{$U\Ra V, A$}
\AxiomC{$B, U\Ra V, A\coimp B$}
\RightLabel{$\coimp$R}
\BinaryInfC{$U\Ra V, A\coimp B$}
\DisplayProof
\end{tabular}
\end{center}
Notice that the antecedent of $\coimp$L rule permits no context. This means that the argument above no longer works since $+\eta+$ is no longer well-defined (the additional multiset in the antecedent would block a $\coimp$L rule in $\eta$). No permutation reduction strategy is apparent in this situation.
\begin{center}
How to adapt cut-elimination to cut-reduction?
\end{center}
For simplicity, read~$X'$ as a single formula in what follows. We propose the following transformation involving a cut on~$X'$.
\begin{equation}\label{cut-reduction-simple}
\text{
\AxiomC{$X' \Ra X'$}
\noLine
\UnaryInfC{$\eta_{[A\imp B/X']}$}
\noLine
\UnaryInfC{$X \Ra Y, X'$}
%
\AxiomC{$X', U'\Ra V'$}
\noLine
\UnaryInfC{$+\pi$}
\noLine
\UnaryInfC{$X', U, C \Ra D$}
\UnaryInfC{$X', U \Ra C\imp D$}
%
\RightLabel{cut}
\BinaryInfC{$X, U\Ra Y, C\imp D$}
\DisplayProof
}
\end{equation}
Observe that $+\pi$ is well-defined also in the bi-intuitionistic setting because the antecedent of every sequent in the featured branch in~$\pi$ contains $A\imp B$ (refer (\ref{right-premise-trace})) and this tells us that no $\coimp$L rule could have occurred on that branch.
When the original cut (\ref{original-cut}) is a topmost non-analytic cut in the given proof it can be shown that $X'$ is necessarily a subformula of the endsequent i.e. the introduced cut is analytic.

Admittedly we have illustrated here a specific case here. The general case will require many analytic cuts and is best seen as constructed from 
the endsequent upwards. Nevertheless, this should already illuminate how a cut-reduction procedure can be obtained as an adaptation of the familiar cut-elimination. Establishing this adaptation in the general case is the main technical content of this paper. 

\section{Proof idea}
The so-called \emph{principal cases} of cut reduction are those where the cut formula is principal in both premises of cut, e.g.
\[
\infer[\cut]{\Gamma\Sa\Delta}
	{
	\infer[\imp_R]{\Gamma\Sa A\imp B,\Delta}
		{
		\infer*[\delta_1]{\Gamma,A\Sa B}{}
		}
	&
	\infer[\imp_L]{\Gamma,A\imp B\Sa\Delta}
		{
		\infer*[\epsilon_1]{\Gamma,A\imp B\Sa A,\Delta}{}
		&
		\infer*[\epsilon]{\Gamma,B\Sa\Delta}{}
		}
	}
\]
In this case the canonical cut reduction is the following:
\[
\infer[\cut]{\Gamma\Sa\Delta}
	{
	\infer[\cut]{\Gamma\Sa A,\Delta}
		{
		\infer[\imp_R]{\Gamma\Sa A\imp B,\Delta}
			{
			\infer*[\delta_1]{\Gamma,A\Sa B}{}
			}
		&
		\infer*[\epsilon_1]{\Gamma,A\imp B\Sa A,\Delta}{}
		}
	&
	\infer[\cut]{\Gamma,A\Sa\Delta}
		{
		\infer*[\delta_1]{\Gamma,A\Sa B}{}
		&
		\infer*[\epsilon]{\Gamma,B\Sa\Delta}{}
		}
	}
\]
The non-principal cases of cut reduction deal with how to achieve the principal case. There are two methods:
\begin{enumerate}
\item Shifting the cut upwards over both premises until one reaches a principal case
\item Globally rewriting the proof such that the cut formula becomes principal in both premises.
\end{enumerate}
The second method works if the rule pertaining to the main connective of the cut formula is invertible. 

Both methods fail in the case of $\BiInt$.  In the following we describe a different method of cut reduction.  This method will not---and cannot---eliminate all cuts, but it will reduce all cuts to analytic ones.

The method is quite similar to the reduction in the principal case, only that we no longer require the cut formula to be principal directly above the cut.  Instead, we trace the cut formula upwards in both branches until it becomes principal:

\[
\infer[\cut]{\Gamma\Sa\Delta}
	{
	\infer*[\delta]{\Gamma\Sa A\imp B,\Delta}
	{
		\infer[\imp_R]{\Gamma'\Sa A\imp B,\Delta'}
			{
			\infer*[\delta_1]{\Gamma',A\Sa B}{}
		}
	}
	&
	\infer*[\epsilon]{\Gamma,A\imp B\Sa\Delta}
	{
	\infer[\imp_L]{\Gamma'',A\imp B\Sa\Delta''}
		{
		\infer*[\epsilon_1]{\Gamma'',A\imp B\Sa A,\Delta''}{}
		&
		\infer*[\epsilon_2]{\Gamma'',B\Sa\Delta''}{}
		}
	}
	}
\]
By making cuts between the subderivations $\delta_1,\epsilon_1$ and $\epsilon_2$ mimicking the principal case reduction one obtains a proof $c(\delta_1,\epsilon_1,\epsilon_2)$ of the sequent $\Gamma'',\Gamma'\Sa\Delta''$ [TODO: picture if necessary]. This is exactly the conclusion of $\imp_L$ in the above proof figure with $\Gamma'$ substituted for $A\imp B$.  The idea is now to extend this substitution to the lower part of the proof, that is, to $\delta$ and $\epsilon$.  Assuming for simplicity that $\Gamma'$ consists of a single formula,  we obtain the following derivation:
\[
\infer[\cut]{\Gamma\Sa\Delta}
	{
	\infer*[\delta\text{ [subst. $\Gamma'$ for $A\imp B$]}]{\Gamma\Sa\Gamma',\Delta}
		{
		\Gamma'\Sa\Gamma',\Delta'
		}
	&
	\infer*[\epsilon\text{ [subst. $\Gamma'$ for $A\imp B$]}]{\Gamma,\Gamma'\Sa\Delta}
		{
		\infer*[c(\delta_1,\epsilon_1,\epsilon_2)]{\Gamma'',\Gamma'\Sa\Delta''}
			{
			}
		}
	}
\]
Herein the cut on $A\imp B$ has been replaced by a cut on $\Gamma'$.  

It is not immediately clear in which sense this proof transformation constitutes a \emph{reduction}.  We will argue for the following: If the cut on $A\imp B$ is the lowermost non-analytic cut in the original proof and if the proof is free from certain redundancies, then
\begin{itemize}
\item either $\Gamma'$ is a proper subformula of $A\imp B$, or
\item $\Gamma'$ is a subformula of $\Gamma\cup\Delta$.
\end{itemize}
In the first case the introduced cut on $\Gamma'$ has smaller degree, and using an inductive argument we may therefore assume that it can be reduced. In the second case, the cut on $\Gamma'$ is analytic, and we just leave it as it is.

A complication arises because analytic cuts in $\delta$ and $\epsilon$ may cease to be analytic after the substitution. But again, we will argue that this is only the case if they were cuts on proper subformulas of $A\imp B$, and thus reducible by induction hypothesis.

Another conceptionally less interesting complication comes from the possibility that there can be multiple instances of $\imp_L$ and $\imp_R$ introducing the cut formula, and from the possibility that $\Gamma'$ contains more than one formula. These are dealt with by \ldots






==> oldpreliminary.tex <==
\begin{figure}[t]
\fbox{
\begin{minipage}{\textwidth}


Initial rule and cut:
\[
\infer[\hyp]{\Gamma,p\Sa p,\Delta}
	{}
\qquad
\infer[\cut]{\Gamma\Sa\Delta}
	{
	\Gamma\Sa A,\Delta
	&
	\Gamma,A\Sa\Delta
	}
\]
Logical rules:
\[
\infer[\top_L]{\Gamma,\top\Sa\Delta}
	{
	\Gamma\Sa\Delta
	}
\qquad
\infer[\top_R]{\Gamma\Sa\top,\Delta}
	{}
\]
\[
\infer[\bot_L]{\Gamma,\bot\Sa\Delta}
	{}
\qquad
\infer[\bot_R]{\Gamma\Sa\bot,\Delta}
	{
	\Gamma\Sa\Delta
	}
\]
\[
\infer[\land_L]{\Gamma,A\land B\Sa\Delta}
	{
	\Gamma,A,B\Sa\Delta
	}
\qquad
\infer[\land_R]{\Gamma\Sa A\land B,\Delta}
	{
	\Gamma\Sa A,\Delta
	&
	\Gamma\Sa B,\Delta
	}
\]
\[
\infer[\lor_L]{\Gamma,A\lor B\Sa\Delta}
	{
	\Gamma,A\Sa\Delta
	&
	\Gamma,B\Sa\Delta
	}
\qquad
\infer[\lor_R]{\Gamma\Sa A\lor B,\Delta}
	{
	\Gamma\Sa A,B,\Delta
	}
\]
\[
\infer[\imp_L]{\Gamma,A\imp B\Sa\Delta}
	{
	\Gamma,A\imp B\Sa A,\Delta
	&
	\Gamma,A\imp B,B\Sa\Delta
	}
\qquad
\infer[\imp_R]{\Gamma\Sa A\imp B,\Delta}
	{
	\Gamma,A\Sa B
	}
\]
\[
\infer[\coimp_L]{\Gamma,A\coimp B\Sa\Delta}
	{
	A\Sa B,\Delta
	}
\qquad
\infer[\coimp_R]{\Gamma\Sa A\coimp B,\Delta}
	{
	\Gamma\Sa A,A\coimp B,\Delta
	&
	\Gamma,B\Sa A\coimp B,\Delta
	}
\]
\end{minipage}}

\caption{The sequent calculus $\BiInt$.}
\label{fig:BiInt}
\end{figure}
\marginpar{maybe move these sentences to the previous section?}
We present our method using the sequent calculus $\BiInt$ for bi-intuitionistic logic as a case study.
%with its history the case study is also interesting in its own.
%
Bi-intuitionistic logic (also known as Heyting–Brouwer logic or as subtractive logic) is the conservative extension of intuitionistic logic with a $\coimp$ connective dual to implication (called coimplication).
%The language of bi-intuitionistic logic extends that of intuitionistic logic through the addition of coimplication~$\coimp$. 
Proposed by Rauzer~\cite{Rau74} the 
calculus $\BiInt$ extends Maehara's multiple-conclusion calculus for intuitionistic logic with suitable rules for $\coimp$. A counterexample to the admissibility of cut stated in~\cite{Rau74}
(and in~\cite{Crolard04}) was later found by Uustalu and Pinto~\cite{PintoU09}. This failure prompted the search for analytic calculi for bi-intuitionistic logic
using extensions of the sequent calculus, including nested sequents~\cite{GorPosTiuAIML},  and  labelled sequents~\cite{PintoU09}. The relations among the two type of calculi have been investigated in \cite{PintoU18}, that left open the problem of finding a syntactic proof of the completeness of 
$\BiInt$ with analytic cuts (see~\cite{AvrLahav,KowOno17} for semantic proofs). 

To simplify our proof of cut-restriction (see Remark~\ref{rem-variant}) we use
a slightly modified (though equivalent) version of $\BiInt$, depicted in
Figure~\ref{fig:BiInt}; here
\begin{itemize}
\item the principal formula in $\hyp$ is an atom~$p$, and 
\item the $\imp_L$ ($\coimp_R$) rule also copies the $A\imp B$ ($A\coimp B$) in the right (left) premise. 
\end{itemize}
\begin{remark}
The pairs of connectives $(\top,\bot)$ and $(\land,\lor)$ are \emph{dual} in classical logic in the sense that the sequent rules for one connective are exactly the `mirror image' of the rule for its dual, a fact already pointed out by Gentzen~\cite{Gen34}. In $\BiInt$ this duality is extended to the pair $(\imp,\coimp)$. The arising symmetry can be captured formally by introducing a formula translation $(\cdot)^\sharp$ that replaces each connective by its dual, where additionally implications are inverted, i.e.\ $(A\imp B)^\sharp=(B^\sharp\coimp A^\sharp)$, $(A\coimp B)^\sharp=(B^\sharp\imp A^\sharp)$. Then exploiting the symmetry of the rules, it is immediate that $\Gamma\Sa\Delta$ is provable in $\BiInt$ iff $\Delta^\sharp\Sa\Gamma^\sharp$ is.
\end{remark}
\marginpar{We need usual preliminaries explaining the difference between rules and instances}
In what follows we will distinguish between
proofs and derivations, referring to 
%Derivations and proofs are defined in the usual way, and with respect to 
$\BiInt$, unless otherwise noted.
\begin{definition}
A \emph{$\BiInt$-derivation} of a sequent $\Gamma\Sa\Delta$ is a tree of sequents rooted in $\Gamma\Sa\Delta$ obtained as rule intances of $\BiInt$.
%such that each interior node together with its node(s) immediately above constitutes a rule instance of $\BiInt$. 
A \emph{$\BiInt$-proof} is a derivation in which all leaves are initial sequents. 
\end{definition}
As usual, the \emph{height} of a proof or derivation is the maximum length of a branch in it.
%
By an easy induction on the formula $A$ we can prove:

begin{lemma}\label{lem:genaxioms}
The sequent $\Gamma,A\Sa A,\Delta$ is derivable in $\BiInt$ without cuts.
\end{lemma}
%\begin{proof}
%By induction on $A$.\qed
%\end{proof}

The following definitions are taken from~\cite{KowOno17}
\begin{definition} %[analytic cut~\cite{KowOno17}]
An instance of the cut rule
\[
\infer[\cut]{\Gamma\Sa\Delta}
	{
	\Gamma\Sa A,\Delta
	&
	\Gamma,A\Sa\Delta
	}
\]
is \emph{analytic} if $A$ is a subformula of $\Gamma\cup\Delta$. A proof is \emph{locally analytic} if every cut in the proof is analytic.
A sequent calculus has the \emph{analytic cut property} if every provable sequent has a locally analytic proof.
\end{definition}

%The \emph{subformula property} of a sequent system states that every sequent provable in the system has a proof in which all occuring formulas are subformulas of the endsequent. 

Any calculus whose rules, except cut, are ``analytic" in the sense that every formula in the premise(s) is a subformula of the end-sequent has the following property: every formula occurring in a locally analytic proof 
%If a proof is locally analytic then it is easily seen\footnote{Implicitly using the observation that every rule of $\BiInt$ that is not the cut-rule is ``analytic" in the sense that every formula in the premise is a subformula of the endsequent} that 
is a subformula of the endsequent. In other words,
the analytic cut property implies the \emph{subformula property}.
This holds, in particular, for $\BiInt$. The converse direction was shown in~\cite[Lem. 4.6]{KowOno17} using an elegant induction argument.




==> proposed.tex <==
Consider the standard bi-intuitionistic sequent calculus with an explicit contraction and weakening rule. In particular, initial sequents are $p \Ra  p$, and the principal formula of $\imp_L$ is not repeated in either premise.

Induction on the size of the cut-formula.

$\blacktriangleright$ Consider an uppermost non-locally analytic cut (we consider multiplicative cuts)
\begin{center}
\AxiomC{$G \Ra  D, A\imp B$}
\AxiomC{$A\imp B, X \Ra  Y$}
\RightLabel{cut}
\BinaryInfC{$G, X \Ra  D, Y$}
\DisplayProof
\end{center}
Call the left premise $\delta$ and the right premise $\epsilon$. Define the derivations $\delta_{A\imp B}$ and $\epsilon_{A\imp B}$ as before although this time there may be multiple predecessors in a sequent since a predecessor in the conclusion of a contraction rule becomes two predecessors in its premise. As before, every predecessor in $\delta_{A\imp B}$ ($\epsilon_{A\imp B}$) is ultimately principal by $\imp_R$  (resp. $\imp_L$ ) (a \textit{critical inference}) or weakening (a \textit{non-critical inference}). 

The \textit{critical antecedent} and \textit{critical succedent} of a critical inference are the sets of formulas in the antecedent and succedent of the conclusion, respectively, omitting (any) predecessors.

E.g. suppose that the following is a critical inference containing exactly two predecessors in its conclusion.
\begin{center}
\AxiomC{$A\imp B, U \Ra  V, A$}
\AxiomC{$A\imp B, B, U \Ra  V, A$}
\RightLabel{$\imp_L$}
\BinaryInfC{$A\imp B, A\imp B, U \Ra  V$}
\DisplayProof
\end{center}
Then its critical antecedent is $U$ and its critical succedent is $V$.

Without loss of generality (the \textit{irredundancy property}) we can assume that neither the derivation $\delta_{A\imp B}$ nor $\epsilon_{A\imp B}$ contains a cut on $A\imp B$ since such a cut can be replaced by a contraction rule e.g.
\begin{center}
\AxiomC{$G' \Ra  D', A\imp B, A\imp B$}
\AxiomC{$A\imp B, G'' \Ra  D''$}
\RightLabel{cut}
\BinaryInfC{$G', G'' \Ra  D', D'', A\imp B$}
\DisplayProof
\end{center}
is replaced by 
\begin{center}
\AxiomC{$G' \Ra  D', A\imp B, A\imp B$}
\RightLabel{c}
\UnaryInfC{$G' \Ra  D', A\imp B$}
\RightLabel{w}
\UnaryInfC{$G', G'' \Ra  D', D'', A\imp B$}
\DisplayProof
\end{center}
Consider the $r^\text{th}$ critical inference in $\delta_{A\imp B}$
\begin{center}
\AxiomC{$A, G_r \Ra  B$}
\RightLabel{$\imp_R$}
\UnaryInfC{$G_r \Ra  A\imp B$}
\DisplayProof
\end{center}
Due to the irredundancy property it we have that every formula in its critical antecedent is a subformula of $G\cup D$ or a proper subformula of $A\imp B$. 

(The proof is the same as before: every formula~$F$ in the critical antecedent is a subformula of $G\Ra D,A\imp B$; if $F=A\imp B$ then under the descendent relation there is some superformula~$F'$ of $A\imp B$ that is a subformula of $G\Ra D,A\imp B$; a contradiction is obtained whether~$F'$ is a subformula of $G\cup D$ or not).

Every critical inference in $\epsilon_{A\imp B}$ has the following form where $A\imp B^{*}$ indicates other predecessors (possibly none) and $\Sigma$ contains no predecessors.
\begin{center}
\AxiomC{$\Sigma, A\imp B^{*} \Ra  A, \Pi$}
\AxiomC{$\Sigma, A\imp B^{*}, B \Ra  \Pi$}
\RightLabel{$\imp_L$}
\BinaryInfC{$\Sigma, A\imp B^{*}, A\imp B \Ra  \Pi$}
\DisplayProof
\end{center}
Obtain $\epsilon_{G_r}$ by simultaneously replacing every predecessor by $G_r$. We can supply proofs for its leaves by weakening with $G_r$ instead of $A\imp B$ (non-critical inferences), and IH applying cuts to smaller formulas (critical inferences). 

Moreover every non-analytic cut in $\epsilon_{G_r}$ must be on a proper subformula of $A\imp B$ (these are cuts that have become non-analytic after the substitution of $G_r$ for $A\imp B$) so those cuts are eliminable by IH. 
Hence we obtain a locally analytic proof of $G_r, U \Ra  V$. 

%Also, since we have replaced every predecessor $A\imp B$ in $\epsilon_{A\imp B}$ with $G_r$, and since the $A\imp B$ appeared in every sequent from leaf to root, so does $G_r$.

Now from $\delta_{A\imp B}$ we can obtain locally analytic proofs of every sequent in the following set by replacing each $G_r \Ra  A\imp B$ with $G_r \Ra  g_r$ ($g_r \in G_r$).
\[
\{ G \Ra  D, g_1, \ldots, g_n | \text{$g_r \in G_r$ for every $r$ ($1\leq r\leq n$)} \}
\]

Suppose that $G_1 = \{ x_1, \ldots, x_m\}$. Then by analytic cut on $\{G \Ra  D, x_1, g_2, \ldots, g_n\}$ and $x_1, \ldots, x_m, U \Ra  V$ and contractions we obtain 
\[
\{x_2, \ldots, x_m, G, U \Ra  D, V, g_2, \ldots, g_n | \text{$g_r \in G_r$ for every $r$ ($2\leq r\leq n$)}\}
\]
By analytic cuts and contractions starting with $\{G \Ra  D, x_2, g_2, \ldots, g_n\}$, \ldots we ultimately obtain $G, U \Ra  D, V, g_2, \ldots, g_n\}$. Proceeding in this way we ultimately obtain a locally analytic proof of $G, U \Ra  D, V$. 

$\blacktriangleright$ Now let's handle the case of the following uppermost non-locally analytic cut
\begin{center}
\AxiomC{$G \Ra  D, A\land B$}
\AxiomC{$A\land B, X \Ra  Y$}
\RightLabel{cut}
\BinaryInfC{$G, X \Ra  D, Y$}
\DisplayProof
\end{center}
Without loss of generality we can assume that neither the derivation $\delta_{A\land B}$ nor $\epsilon_{A\land B}$ contains a cut on $A\land B$ since such a cut can be replaced by a contraction rule e.g.
\begin{center}
\AxiomC{$G' \Ra  D', A\land B, A\land B$}
\AxiomC{$A\land B, G'' \Ra  D''$}
\RightLabel{cut}
\BinaryInfC{$G', G'' \Ra  D', D'', A\land B$}
\DisplayProof
\end{center}
is replaced by 
\begin{center}
\AxiomC{$G' \Ra  D', A\land B, A\land B$}
\RightLabel{c}
\UnaryInfC{$G' \Ra  D', A\land B$}
\RightLabel{w}
\UnaryInfC{$G', G'' \Ra  D', D'', A\land B$}
\DisplayProof
\end{center}
%\textbf{Morever we can assume a further irredundancy property: $\delta_{A\land B}$ does not contain a cut on either $A$ or on $B$.}
%To see this, consider a topmost cut of the latter (we have illustrated below when that cut is on $B$), and consider the leaves in $\delta_{A\land B}$ above the left premise of that cut.
%\begin{center}
%\AxiomC{for clarity, only critical inferences shown below}
%\noLine
%\UnaryInfC{$\left\{ \frac{G_r\Ra A, A\land B^{*}, D_r\quad G_r\Ra B, A\land B^{*}, D_r}{G_r\Ra A\land B, A\land B^{*}, D_r} \right\}$}
%\noLine
%\UnaryInfC{$\vdots$ no cuts on $A$, $B$, $A\land B$}
%\noLine
%\UnaryInfC{$L_{1}\Ra B, A\land B, A\land B^{*}, M_{1}$}
%%
%\AxiomC{$B, L_{2}\Ra A\land B^{**}, M_{2}$}
%\RightLabel{cut}
%\BinaryInfC{$L_{1}, L_{2}\Ra A\land B, A\land B^{*}, A\land B^{**}, M_{1}, M_{2}$}
%\noLine
%\UnaryInfC{$\vdots$}
%\noLine
%\UnaryInfC{$G\Ra D, A\land B$}
%\DisplayProof
%\end{center}
%Replace the cut on~$B$ with the following.
%\begin{center}
%\AxiomC{$\{ G_r\Ra A, A\land B^{*}, D_r \}$}
%\noLine
%\UnaryInfC{$\vdots$}
%\noLine
%\UnaryInfC{$L_{1}\Ra A, A\land B^{*}, M_{1}$}
%\RightLabel{w}
%\UnaryInfC{$L_{1}\Ra A, A\land B, A\land B^{*}, M_{1}$}
%%
%\AxiomC{$\vdots$}
%\noLine
%\UnaryInfC{$L_{1}\Ra B, A\land B, A\land B^{*}, M_{1}$}
%\RightLabel{$\land_L$}
%\BinaryInfC{$L_{1}\Ra A\land B, A\land B, A\land B^{*}, M_{1}$}
%\RightLabel{w,c}
%\UnaryInfC{$L_{1}, L_{2}\Ra A\land B, A\land B^{*}, A\land B^{**}, M_{1}, M_{2}$}
%\DisplayProof
%\end{center}

Finally: every conclusion $G' \Ra  D', A\land B$ of a leaf in $\delta_{A\land B}$ can be replaced with $G' \Ra  D', A$ in the obvious ways to obtain a proof of $G \Ra  D, A$. Any non-analytic cut in this proof must be on a subformula of $B$ (it cannot be on $A\land B$ by the irredundancy property). Hence we get a locally analytic proof of $G \Ra  D, A$ by eliminating all non-analytic cuts by IH. Similarly we get a locally analytic proof of $G \Ra  D, B$. 
Replacing $A\land B$ with $A,B$ in the obvious way plus the irredundancy property immediately yields a locally analytic proof of $\epsilon_{A\land B}$.

The result now follows by appealing to IH for a cut on $A$, and then on $B$.
